Snowmass 2021 White Paper on Upgrading SuperKEKB with a Polarized Electron Beam: Discovery Potential and Proposed Implementation

Upgrading the SuperKEKB electron-positron collider with polarized electron beams opens a new program of precision physics at a center-of-mass energy of 10.58 GeV. This white paper describes the physics potential of this `Chiral Belle' program. It includes projections for precision measurements of $\sin^2\theta_W$ that can be obtained from independent left-right asymmetry measurements of $e^+e^-$ transitions to pairs of electrons, muons, taus, charm and b-quarks. The $\sin^2\theta_W$ precision obtainable at SuperKEKB will match that of the LEP/SLC world average, but at the centre-of-mass energy of 10.58 GeV. Measurements of the couplings for muons, charm, and $b$-quarks will be substantially improved and the existing $3\sigma$ discrepancy between the SLC $A_{LR}$ and LEP $A_{FB}^b$ measurements will be addressed. Precision measurements of neutral current universality will be more than an order of magnitude more precise than currently available. As the energy scale is well away from the $Z^0$-pole, the precision measurements will have sensitivity to the presence of a parity-violating dark sector gauge boson, $Z_{\rm dark}$. The program also enables the measurement of the anomalous magnetic moment $g-2$ form factor of the $\tau$ to be made at an unprecedented level of precision. A precision of $10^{-5}$ level is accessible with 40~ab$^{-1}$ and with more data it would start to approach the $10^{-6}$ level. This technique would provide the most precise information from the third generation about potential new physics explanations of the muon $g-2$ $4\sigma$ anomaly. Additional $\tau$ and QCD physics programs enabled or enhanced with having polarized electron beams are also discussed in this White Paper. This paper includes a summary of the path forward in R&D and next steps required to implement this upgrade and access its exciting discovery potential.

==> Acknowlegements.tex <==
{ \bf Acknowledgements}
This work was supported in part by the following funding sources:
U.S. Department of Energy contract DE-AC05-06OR23177, under which Jefferson Science Associates LLC manages and operates Jefferson Lab. AA also acknowledges support from DOE contract DE-SC0008791.
A.S. acknowledges support from the European Commission through the Marie Sklodowska-Curie Action SQuHadron (grant agreement ID: 795475); Brookhaven Science Associates, LLC under Contract No. DE-SC0012704; Science Committee of the Republic of Armenia Grant No.  18T-1C180; Australian ResearchCouncil and research grant Nos.  DP180102629, DP170102389, DP170102204, DP150103061,FT130100303, and FT130100018; Austrian Federal Ministry of Education, Science and Re-search,  and  Austrian  Science  Fund  No.   P  31361-N36;  Natural  Sciences  and  Engineering Research Council of Canada, Compute Canada and CANARIE; Chinese Academy of Sciences and research grant No.  QYZDJ-SSW-SLH011, National Natural Science Foundation of China and research grant Nos.  11521505, 11575017, 11675166, 11761141009, 11705209,and 11975076, LiaoNing Revitalization Talents Program under contract No.  XLYC1807135,Shanghai Municipal Science and Technology Committee under contract No.  19ZR1403000,Shanghai Pujiang Program under Grant No.  18PJ1401000, and the CAS Center for Excellence in Particle Physics (CCEPP); the Ministry of Education, Youth and Sports of the Czech Republic  under  Contract  No.  LTT17020  and  Charles  University  grants  SVV  260448  and GAUK 404316; European Research Council, 7th Framework PIEF-GA-2013-622527, Horizon 2020 Marie Sklodowska-Curie grant agreement No.  700525 ‘NIOBE,’ and Horizon 2020Marie Sklodowska-Curie RISE project JENNIFER2 grant agreement No.  822070 (European grants); L’Institut National de Physique Nucl\'eaire et de Physique des Particules (IN2P3) duCNRS (France); BMBF, DFG, HGF, MPG, AvH Foundation, and Deutsche Forschungsge-meinschaft (DFG) under Germany’s Excellence Strategy – EXC2121 “Quantum Universe”’–  390833306  (Germany);  Department  of  Atomic  Energy  and  Department  of  Science  and Technology (India); Israel Science Foundation grant No.  2476/17 and United States-Israel Binational  Science  Foundation  grant  No.   2016113;  Istituto  Nazionale  di  Fisica  Nucleare and the research grants BELLE2; Japan Society for the Promotion of Science, Grant-in-Aid for Scientific Research grant Nos.  16H03968,  16H03993,  16H06492,  16K05323,  17H01133,17H05405,  18K03621,  18H03710,  18H05226,  19H00682,  26220706,  and  26400255,  the  National Institute of Informatics, and Science Information NETwork 5 (SINET5), and the Ministry of Education, Culture, Sports, Science, and Technology (MEXT) of Japan; National Research Foundation (NRF) of Korea Grant Nos.  2016R1D1A1B01010135, 2016R1D1A1B-02012900, 2018R1A2B3003643, 2018R1A6A1A06024970, 2018R1D1A1B07047294, 2019K1-A3A7A09033840,  and  2019R1I1A3A01058933,  Radiation  Science  Research  Institute,  Foreign  Large-size  Research  Facility  Application  Supporting  project,  the  Global  Science  Experimental  Data  Hub  Center  of  the  Korea  Institute  of  Science  and  Technology  Information  and  KREONET/GLORIAD;  Universiti  Malaya  RU  grant,  Akademi  Sains  Malaysia and  Ministry  of  Education  Malaysia;  Frontiers  of  Science  Program  contracts  FOINS-296,22 CB-221329, CB-236394, CB-254409, and CB-180023, and SEP-CINVESTAV research grant237 (Mexico); the Polish Ministry of Science and Higher Education and the National Science  Center;  the  Ministry  of  Science  and  Higher  Education  of  the  Russian  Federation,Agreement 14.W03.31.0026; University of Tabuk research grants S-1440-0321, S-0256-1438,and S-0280-1439 (Saudi Arabia);  Slovenian Research Agency and research grant Nos.  J1-9124  and  P1-0135;  Agencia  Estatal  de  Investigacion,  Spain  grant  Nos.   FPA2014-55613-P  and  FPA2017-84445-P,  and  CIDEGENT/2018/020  of  Generalitat  Valenciana;  Ministryof  Science  and  Technology  and  research  grant  Nos.   MOST106-2112-M-002-005-MY3  and MOST107-2119-M-002-035-MY3, and the Ministry of Education (Taiwan); Thailand Center of Excellence in Physics;  TUBITAK ULAKBIM (Turkey);  Ministry of Education and Science  of  Ukraine;  the  US  National  Science  Foundation  and  research  grant  Nos.   PHY-1807007 and PHY-1913789, and the US Department of Energy and research grant Nos.  DE-AC06-76RLO1830,  DE-SC0007983,  DE-SC0009824,  DE-SC0009973,  DE-SC0010073,  DE-SC0010118, DE-SC0010504, DE-SC0011784, DE-SC0012704; and the National Foundation for  Science  and  Technology  Development  (NAFOSTED)  of  Vietnam  under  contract  No103.99-2018.4

==> B2UpgradeWP-IntroParagraphonChiralBelle.tex <==
\topmargin -.85in
\setlength{\textwidth}{7.in}
\setlength{\textheight}{9.7in}
\setlength{\oddsidemargin}{-0.25in}
\setlength{\evensidemargin}{-0.25in}


\pagestyle{empty}
\usepackage{amsmath}
\usepackage{xspace}
\usepackage{hyperref}

\usepackage{graphicx}
\usepackage{graphicx}

\usepackage{booktabs}
\usepackage{caption}
\usepackage{subcaption}


\usepackage{float}

\usepackage[utf8]{inputenc}
%\usepackage{natbib}
\usepackage{graphicx}
\usepackage{verbatim} %enables block comments

\graphicspath{{Plots/}}


\begin{document}

The SuperKEKB e$^+$e$^-$ collider operating at a centre-of-mass energy of 10.58~GeV,
with its high design luminosity of $8\times 10^{35}$~cm$^{-2}$~s$^{-1}$,
 can access new windows for discovery with the Belle~II 
experiment if it is upgraded to have a longitudinally polarized electron beam.
 The target integrated luminosity for SuperKEKB/Belle~II is 50~ab$^{-1}$\cite{BelleIITDR}
 and currently Belle~II is projected to collect that amount of data, which will not have beam polarization without an upgrade to SuperKEKB, by 2027.
 Upgrading SuperKEKB to have electron beams with left and right longitudinal polarization of approximately 70\% at the Belle~II interaction point creates 
 a unique and versatile facility for probing new physics with precision electroweak measurements that no other experiments, current or planned, 
 can achieve.
 
 \end{document}
 

==> SKB-B2-PolUpgradeGroup.tex <==
%\footnote{
U.~Wienands (Argonne National Lab, USA);
M.~Hoferichter (Univ. of Bern, Switzerland);
C.~Hearty (Univ. British Columbia, Canada)
I.~A.~Koop, A.~V.~Otboev, Yu.~M.~Shatunov (BINP, Novosibirsk, Russia);
B.~Parker (Brookhaven National Lab, USA);
A.~Schwartz (Univ. of Cincinnati, USA);
A.~Vossen (Duke Univ., USA);
A.~Accardi (Hampton U. and Jefferson Lab, USA)
M.~Kuriki, Z.~Liptak (Hiroshima Univ., Japan);
F.~R.~Le~Diberder, A.~Martens, K.~Trabelsi, F.~Zomer
(IJCLab, France);
D.~Zhou (KEK, Japan) 
Sw.~Banerjee (Univ. of Louisville, USA); 
W.~Deconinck, M.~Gericke, J.~Mammei  (Univ. of Manitoba, Canada); 
A.~Signori (Univ. of Pavia and INFN, Italy);
R.~Baartman, T.~Planche (TRIUMF, Canada);
A.~Beaubien, T.~Junginger, C.~Miller, K.~Moorthy Y.~Peng, J.~M.~Roney (Univ. of Victoria, Canada)
%}

==> SuperKEKB_ePolarization.tex <==
% Please make sure you insert your
% data according to the instructions in PoSauthmanual.pdf
%\documentclass{PoS}

\title{Electroweak Physics with Polarized Electron Beams in a SuperKEKB Upgrade}

\ShortTitle{EW Physics with Polarized e$^-$ Beams in a SuperKEKB Upgrade}

\author{\speaker{J. Michael Roney}
        \thanks{Critical work by Uli Wienands and Demin Zhou developing the accelerator concepts needed for a potential
beam polarization upgrade to SuperKEKB is acknowledged. Calculations conducted by  A.~Aleksejevs, S.~Barkanova and V.~Zykunov confirm
the sensitivity of $A_{LR}$ to the neutral current couplings at NLO.}\\
        University of Victoria\\
        E-mail: \email{mroney@uvic.ca}}

%\author{Another Author\\
%        Affiliation\\
%        E-mail: \email{...}}

\abstract{A potential upgrade of the SuperKEKB e$^+$e$^-$ collider with a polarized  electron beam
 will open a new program of precision electroweak physics at the centre-of-mass energy of the $\Upsilon$(4S) and is currently being considered.
 These measurements include $\sin^2\theta_W$ obtained via left-right asymmetry measurements of
 e$^+$e$^-$ transitions to pairs of electrons, muons, taus, charm and b-quarks.
 The precision obtainable at SuperKEKB will match that of the LEP/SLC world average but at the centre-of-mass energy of 10.58~GeV,
 thereby probing the neutral current couplings with unprecedented precision at a new energy scale sensitive to the running of the couplings.
 World average measurements of the individual neutral current vector coupling constants to b- and c-quarks and muons in particular will be
 substantially improved and the residual $3\sigma$ discrepancy between the SLC $A_{LR}$ and LEP $A_{FB}^b$
 measurements will be addressed. This paper will include a discussion of the necessary upgrades to SuperKEKB.
 This program opens an exciting new window in searches for physics beyond the standard model.}

\FullConference{XXIX International Symposium on Lepton Photon Interactions at High Energies - LeptonPhoton2019\\
		August 5-10, 2019\\
		Toronto, Canada}


\begin{document}
The SuperKEKB e$^+$e$^-$ collider operating at a centre-of-mass energy of 10.58~GeV,
with its high design luminosity of $8\times 10^{35}$~cm$^{-2}$~s$^{-1}$,
 can access new windows for discovery with the Belle~II 
experiment if it is upgraded to have a longitudinally polarized electron beam.
 The target integrated luminosity for SuperKEKB/Belle~II is 50~ab$^{-1}$\cite{BelleIITDR}
 and currently Belle~II is projected to collect that amount of data, which will not have beam polarization without an upgrade to SuperKEKB, by 2027.
 Upgrading SuperKEKB to have electron beams with left and right longitudinal polarization of approximately 70\% at the Belle~II interaction point creates 
 a unique and versatile facility for probing new physics with precision electroweak measurements that no other experiments, current or planned, 
 can achieve.

 In particular, a data sample of 20~ab$^{-1}$ with a polarized electron beam enables Belle~II to measure the weak neutral current vector coupling 
 constants of the $b$-quark, $c$-quark and muon at significantly higher precision than any previous experiment. 
 With 40~ab$^{-1}$ of polarized beam data, the precision of
 the vector couplings to the tau and electron can be measured at a level comparable to current world averages, which are dominated by
 LEP and SLD measurements at the Z$^0$-pole.

 Within the framework of the Standard Model (SM) these measurements of $g_V^f$, the neutral current vector coupling for fermion $f$,
 can be used to determine the weak mixing angle, $\theta_W$, 
through the relation: $g_V^f = T_3^f - 2Q_f \sin^2\theta_W$, where $T_3^f$ is the $3^{rd}$ component of weak isospin of fermion $f$,
 $Q_f$ is its electric charge in units of electron charge and
the notational conventions of Reference~\cite{LEPSLDReport2006} are used.


As described in Reference~\cite{SuperBTDR},
with polarized electron beams an e$^+$e$^-$ collider at 10.58~GeV can
 determine $g_V^f$  by measuring the left-right asymmetry, $A_{LR}^f$, for each identified final-state fermion-pair in the process
$e^+e^- \rightarrow f \overline{f}$:
\begin{equation}
 A_{LR}^f = \frac{ \sigma_L - \sigma_R}{\sigma_L + \sigma_R} = \frac{s G_F }{\sqrt{2} \pi \alpha Q_f} g_A^e g_V^f \langle Pol \rangle
\end{equation}
where $g_A^e = T_3^e = -\frac{1}{2}$ is the neutral current axial coupling of the electron, $G_F$ is the Fermi coupling constant,
$s$ is the square of the centre-of-mass energy, and 
\begin{equation}
\langle Pol \rangle =\frac{1}{2} \left[ \left(\frac{N_{eR}-N_{eL}}{N_{eR}+N_{eL}}\right)_{\mathbf R} -
 \left(\frac{N_{eR}-N_{eL}}{N_{eR}+N_{eL}}\right)_{\mathbf L} \right]
\end{equation}
is the average electron beam polarization, where  $N_{eR}$ is the number of right-handed electrons and $N_{eL}$
 the number of left-handed electrons in the event samples where the electron beam bunch is left polarized or right polarized,
 as indicated by the `${\mathbf L}$' and `${\mathbf R}$' subscripts. 
 These asymmetries arise from $\gamma-Z$ interference and although the
 SM asymmetries are small ($-6\times 10^{-4}$ for the leptons, $-5\times 10^{-3}$ for charm and
 $-2\%$ for the $b$-quarks), unprecedented precisions can be achieved 
 because of the combination of both the high luminosity of SuperKEKB and a $70\%$ beam polarization measured with a precision of better than $\pm 0.5\%$.
Note that higher order corrections are ignored here for simplicity, although studies at higher orders have recently begun~\cite{Aleskejevs}.

 The upgrade to SuperKEKB involves three hardware projects:\\
1)  A low-emittance polarized electron source in which 
  the electron beams would be produced via a polarized laser illuminating a ``strained lattice'' GaAs photocathode
 as was done for SLD~\cite{LEPSLDReport2006}. The source would produce longitudinally polarized electron bunches whose spin would be rotated to be transversely polarized before it
 enters the SuperKEKB electron storage ring;\\
2) A pair of spin-rotators, one positioned before and the other after the interaction region, to rotate the spin to longitudinal
 prior to collisions and back to transverse following collisions. One configuration under consideration for the spin-rotator is a
  combined function magnet that replaces an existing dipole in the SuperKEKB electron beam lattice with a superconducting
  magnet that has both a dipole and solenoid~\cite{UliWienands} as well as six skew quads.
 The challenge is to design the rotators to minimize couplings between vertical and horizontal planes and to address higher order and chromatic effects 
 in the design to ensure the luminosity is not degraded; \\
3) A Compton polarimeter that measures the beam polarization before the beam enters the interaction region.


 The high precisions are possible at such an upgraded SuperKEKB
 because with 20~ab$^{-1}$ of data Belle~II can identify between $10^9$ and $10^{10}$ final-state pairs of b-quarks, c-quarks, taus, muons and electrons
 with high purity and reasonable signal efficiency,
 and because all detector-related systematic errors can be made to cancel by flipping
 the laser polarization from ${\mathbf R}$ to ${\mathbf L}$ in a random, but known, pattern as collisions occur.
 $\langle Pol \rangle$ would be measured in two ways. The first method uses a Compton polarimeter, which can be expected to have an absolute
 uncertainty at the Belle~II interaction point of less than $1\%$ and
 provides a `bunch-by-bunch' measurement of $\left(\frac{N_{eR}-N_{eL}}{N_{eR}+N_{eL}}\right)_{\mathbf R}$
 and $\left(\frac{N_{eR}-N_{eL}}{N_{eR}+N_{eL}}\right)_{\mathbf L}$. The uncertainty will be dominated by the need to predict the polarizatoin loss
 from the Compton polarimeter to the interaction point. The second method 
 measures the polar angle dependence of the polarization of $\tau$-leptons produced in $e^+e^- \rightarrow \tau^+ \tau^-$ events using the kinematic distributions of the
 decay products of the $\tau$ separately for the ${\mathbf R}$ and ${\mathbf L}$ data samples.
 The forward-backward asymmetry of the tau-pair polarization is linearly dependent on $\langle Pol \rangle$ and therefore
 can be used to determine $\langle Pol \rangle$ to $0.5\%$ at the Belle~II interaction point in a manner entirely independent of the Compton polarimeter. 
 The $\tau$ polarization forward-backward asymmetry method avoids the uncertainties associated with tracking the polarization losses to the interaction point and also
 automatically accounts for any residual positron polarization that might be present. In addition, it automatically provides a luminosity-weighted beam
 polarization measurement.

 Table~\ref{Table-measurements} provides the sensitivities to electroweak parameters expected with polarized electron beams in an upgraded SuperKEKB from
$e^+e^- \rightarrow b \bar{b}$, $e^+e^- \rightarrow c \bar{c}$, $e^+e^- \rightarrow \tau^+ \tau^-$, $e^+e^- \rightarrow \mu^+ \mu^-$, 
and $e^+e^- \rightarrow e^+ e^-$ events selected by Belle~II. From this information the precision on the b-quark, c-quark and muon neutral current vector couplings 
will improve by a factor of four, seven and five, respectively, over the current world average values\cite{LEPSLDReport2006} with 20~ab$^{-1}$ of polarized data.

This is of particular importance for $g^b_V$, where the measurement of -0.3220$\pm$0.0077 is  2.8$\sigma$ higher than the SM value of -0.3437~\cite{LEPSLDReport2006}.
That discrepancy arises from the 3$\sigma$ difference between the SLC $A_{LR}$ measurements and LEP $A^b_{FB}$ measurements of $\sin^2\theta_W^{eff}$. 
A measurement of $g^b_V$ at an upgraded SuperKEKB that is four times more precise and which avoids the hadronization uncertainties that are a significant component
 of the uncertainties of the measurement of the forward-backward asymmetry at LEP, or any other forward-backward asymmetry measurement
 using on-shell $Z^0$ bosons, will be able to definitively resolve whether or not this is
a statistical fluctuation or a first hint of a genuine breakdown of the SM. 

\begin{figure}
%\begin{figure*}[h]
\centering
\includegraphics[width=0.49\textwidth]{sin2thetaW.pdf}
\raisebox{0.1\height}{\includegraphics[width=0.49\textwidth]{Zdark-sin2thetaWvsQ.pdf}}
%\includegraphics[width=135mm]{sin2thetaW.pdf}
\caption{Left: Determination of $\sin^2\theta_W$ at present and future experimental facilities as a function of energy scale,
 adapted from \cite{ErlerPDG2018}. Right: Dark blue band shows Q$^2$-dependent shift in $\sin^2\theta_W$ caused by a 15~GeV mass dark Z,
 adapted from \cite{Davoudiasl}.}
 \label{fig:sin2thetaW}
\end{figure}


\begin{table*}[h]
\begin{center}
\begin{tabular}{|l|c|c|r|c|c|c|}
\hline
Final State & $A_{LR}^{SM}$ &  Relative $A_{LR}$  &$g^f_V$  & $\sigma(g^f_V)$  & $\sigma(g^f_V)$  & $\sigma(s^2 \theta_W)$ \\
Fermion     &               &   Error (\%)& W.A.\cite{LEPSLDReport2006}  & (20~ab$^{-1}$) & (40~ab$^{-1}$) & (40~ab$^{-1}$)             \\ 
\hline 
 b-quark     &  -0.020      &  0.5                &  -0.3220               &   0.002          &   0.002          & 0.003 \\
 (eff.=0.3)  &              &                     & $\pm 0.0077$           &improves x4        &                  &       \\
 \hline
 c-quark     &  -0.005      &  0.5                &  +0.1873               &   0.001          &   0.001          & 0.0007 \\
 (eff.=0.3)  &              &                     &  $\pm 0.0070$          &  improves x7      &                  &        \\
 \hline
 tau         & -0.0006      &  2.3                &  -0.0366               &   0.0008         &   0.0006         &  0.0003 \\
 (eff.=0.25) &              &                     &  $\pm 0.0010$          &                  &                  &       \\ 
 \hline
 muon        & -0.0006      &  1.5                &  -0.03667              &   0.0005         &   0.0004         & 0.0002 \\
 (eff.=0.5)  &              &                     &  $\pm 0.0023$          &   improves x5     &                  &       \\
 \hline
 electron    & -0.0006      &  1.2                &  -0.3816               &   0.0004         &   0.0003         & 0.0002 \\
(1~nb acceptance)&          &                     &  $\pm 0.00047$         &                  &                  &       \\
 \hline
\end{tabular}
\caption{For each fermion pair cleanly identifiable in Belle~II for the given efficiency in column~1: column~2 gives
the SM value of $A_{LR}$; column~3, the expected 
relative error on $A_{LR}$ based on based on 20~ab$^{-1}$
and  a beam polarization at Belle~II of 70\% with an error of $\pm0.5\%$;
column~4, the current world average value of its neutral current vector coupling;
column~5, the projected error on $g_V^f$ with 20~ab$^{-1}$ of data; 
column~6, the projected error on $g_V^f$ with 40~ab$^{-1}$ of data; and 
column~7, the projected SuperKEKB/Belle~II error on $\sin^2\theta_W^{eff}$ with 40~ab$^{-1}$ of polarized e$^-$ beam data.
}
\label{Table-measurements}
\end{center}
\end{table*}



Table~\ref{Table-measurements} also indicates the uncertainties on $\sin^2\theta_W^{eff}$ that can be achieved with
 40~ab$^{-1}$ of polarized beam data - the combined uncertainty at Belle~II would be comparable to the Z$^0$ world average measured uncertainty
of $\pm 0.00016$ from LEP and SLD\cite{LEPSLDReport2006} but made at a significanlty lower energy scale.
Figure~\ref{fig:sin2thetaW}(left) shows the determinations of $\sin^2\theta_W$ as a function of energy scale at present and future experimental
facilities including SuperKEKB upgraded with a polarized electron beam delivering 40~ab$^{-1}$ of data to Belle~II.
 


This electroweak program with polarized electron beams in SuperKEKB
 would provide the highest precision tests of neutral current vector coupling universality.
In addition, right-handed $b$-quark couplings to the $Z$ can  be experimentally
probed with high precision at Belle~II with polarized beams.  Also, measurements with the
projected precision will enable Belle~II to probe parity violation
induced by the exchange of heavy particles such as a
hypothetical TeV-scale $Z^\prime$ boson(s). If such bosons only couple
to leptons they will not be produced at the LHC.  Moreover, the
SuperKEKB machine will have a unique possibility to probe parity
violation in the lepton sector mediated by light and very weakly
coupled particles often referred to as ``Dark Forces''.
Such forces have been entertained as a possible connecting link between normal and dark
matter \cite{Pospelov:2008jd,ArkaniHamed:2008qn}. 
SuperKEKB with polarization would be uniquely sensitivity to ``Dark Sector'' parity violating light neutral gauge
bosons, especially when $Z_{dark}$ is
 off-shell and with a mass between roughly 10 and 35~GeV \cite{Davoudiasl} or even up to the Z$^0$ pole,
 or couples more to the 3rd generation (see Figure~\ref{fig:sin2thetaW}(right)).

The enhancement of
parity violation in the muon sector has been an automatic consequence
of some models \cite{Batell:2011qq} that aim at explaining the
unexpected result for the recent Lamb shift measurement in muonic
hydrogen \cite{Pohl:2010zza}. The left-right asymmetry of the $e^-e^+
\to \mu^-\mu^+$ in such models is expected to be enhanced at
low-to-intermediate energies, and SuperKEKB with polarized beams may provide a
conclusive test of such models, as well as impose new constraints on a
parity-violating dark sector.

%An electron beam polarization upgrade at SuperKEKB  opens a
%an exciting and unique discovery window with precision electroweak physics. 
% A growing international team  has begun to study the feasibility of such an upgrade with the
%goal to begin taking Belle~II data with polarized SuperKEKB electron beams in the mid-2020's. 

%\begin{acknowledgments}
%The collaboration with Uli Wienands and Demin Zhou have been essential for developing the accelerator concepts needed for a potential
%beam polarization upgrade to SuperKEKB. Calculations conducted by  A.~Aleksejevs, S.~Barkanova and V.~Zykunov confirm
%the sensitivity of $A_{LR}$ to the neutral current couplings at NLO.
%\end{acknowledgments}

%\section{...}

\begin{thebibliography}{99}
\bibitem{BelleIITDR} 
T.~Abe {\em et al.} Belle II Technical Design Report, KEK Report 2010-1,
Edited by Z.~Dolezal and S.~Uno, arXiv:1011.0352 (2010).
\bibitem{LEPSLDReport2006} 
ALEPH and DELPHI and L3 and OPAL and SLD Collaborations and LEP Electroweak Working Group and SLD Electroweak Group and SLD Heavy Flavour Group (S. Schael et al.),
`` Precision electroweak measurements on the Z$^0$ resonance'', Phys.Rept. 427 (2006) 257-454.
\bibitem{SuperBTDR} M.~Baszczyk {\em et al.} (SuperB Collaboration), ``SuperB Technical Design Report'', INFN-13-01/PI, LAL 13-01, SLAC-R-1003,
 arXiv:1306.5655 [physics.ins-det].
\bibitem{Aleskejevs} A.~Aleksejevs, S.~Barkanova, C.~Miller, J.M.~Roney and V.~Zykunov,
``NLO Radiative Corrections for Forward-Backward and Left-Right Asymmetries at a B-Factory'', arXiv:1801.08510.
\bibitem{ErlerPDG2018} J.~Erler and A. Freitas ``ElectroweakModel and Constraints on New Physics'' 
 in M. Tanabashi {\em et al.} (Particle Data Group), Phys.~Rev.~D{\bf 98}, 030001 (2018);
 J.~Benesch {\em et al.} (Moller Collaboration), ``The MOLLER Experiment: An Ultra-Precise Measurement of the Weak Mixing Angle Using M{\o}ller Scattering'',
JLAB-PHY-14-1986, arXiv:1411.4088v2 [nucl-ex] 2014;
D.~ Becker {\em  et al.}  ``The P2 experiment'', arXiv:1802.04759 [nucl-ex] 2018.
\bibitem{UliWienands} Uli Wienands, private communication
\bibitem{Pospelov:2008jd} M.~Pospelov and A.~Ritz, ``Astrophysical Signatures of Secluded Dark Matter'', Phys. Lett. B671:391–397,
2009.
\bibitem{ArkaniHamed:2008qn} N.~Arkani-Hamed, D.~P.~Finkbeiner, T.~R.~Slatyer, and N.~Weiner, ``A Theory of Dark Matter'', Phys. Rev. D79:015014, 2009.
\bibitem{Batell:2011qq} B.~Batell, D.~McKeen, and M.~Pospelov,
``New Parity-Violating Muonic Forces and the Proton Charge Radius'', Phys.Rev.Lett. 107:011803, 2011.
arXiv:1103.0721 [hep-ph].
\bibitem{Pohl:2010zza} R.~Pohl, A.~Antognini, F.~Nez, F.~D.~Amaro, F.~Biraben, et al., ``The size of the proton'', Nature 466:213–216, 2010.
\bibitem{Davoudiasl} H.~Davoudiasl, H.~S.~Lee and W.~J.~Marciano, Phys.Rev. D 92, no. 5, 055005 (2015)

\end{thebibliography}

\end{document}


==> USBelle2.tex <==
 
 \vskip0.30in \Large on behalf of the U.S. Belle II Collaboration

% Authors -------------------------------------------------
  \author[1]{D.~M.~Asner}\affil[1]{Brookhaven National Laboratory, Upton, New York 11973}
  \author[2]{Sw.~Banerjee}\affil[2]{University of Louisville, Louisville, Kentucky 40292}
  \author[3]{J.~V.~Bennett}\affil[3]{University of Mississippi, University, Mississippi 38677}
  \author[4]{G.~Bonvicini}\affil[4]{Wayne State University, Detroit, Michigan 48202}
  \author[5]{R.~A.~Briere}\affil[5]{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213}
  \author[6]{T.~E.~Browder}\affil[6]{University of Hawaii, Honolulu, Hawaii 96822}
  \author[2]{D.~N.~Brown}
  \author[7]{C.~Chen}
  \author[4]{D.~Cinabro}
  \author[7]{J.~Cochran}\affil[7]{Iowa State University, Ames, Iowa 50011}
  \author[3]{L.~M.~Cremaldi}
  \author[1]{A.~Di~Canto}
  \author[6]{K.~Flood}
  \author[8]{B.~G.~Fulsom}\affil[8]{Pacific Northwest National Laboratory, Richland, Washington 99352}
  \author[9]{R.~Godang}\affil[9]{University of South Alabama, Mobile, Alabama 36688}
  \author[3]{M.~Hern\'{a}ndez~Villanueva}
  \author[10]{W.~W.~Jacobs}\affil[10]{Indiana University, Bloomington, Indiana 47408}
  \author[1]{D.~E.~Jaffe}
  \author[11]{K.~Kinoshita}\affil[11]{University of Cincinnati, Cincinnati, Ohio 45221}
  \author[3]{R.~Kroeger}
  \author[12]{R.~Kulasiri}\affil[12]{Kennesaw State University, Kennesaw, Georgia 30144}
  \author[1]{P.~J.~Laycock}
  \author[6]{K.~A.~Nishimura}
  \author[1]{B.~Parker} 
  \author[13]{T.~K.~Pedlar}\affil[13]{Luther College, Decorah, Iowa 52101}
  \author[14]{L.~E.~Piilonen}\affil[14]{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061}
  \author[7]{S.~Prell}
  \author[15]{J.~M.~Roney}\affil[15]{University of Victoria, Victoria, British Columbia, V8W 3P6, Canada}
  \author[16]{C.~Rosenfeld}\affil[16]{University of South Carolina, Columbia, South Carolina 29208}
  \author[17]{A.~Rostomyan}\affil[17]{Deutsches Elektronen–Synchrotron, 22607 Hamburg, Germany}
  \author[3]{D.~A.~Sanders}
  \author[18]{V.~Savinov}\affil[18]{University of Pittsburgh, Pittsburgh, Pennsylvania 15260}
  \author[11]{A.~J.~Schwartz}
  \author[8]{J.~Strube}
  \author[3]{D.~J.~Summers}
  \author[6]{S.~E.~Vahsen}
  \author[6]{G.~S.~Varner}
  \author[19]{A.~Vossen}\affil[19]{Duke University, Durham, North Carolina 27708}
  \author[20]{U.~Wienands}\affil[20]{Argonne National Laboratory, Lemont, Illinois 60439}
  \author[8]{L.~Wood}
  \author[21]{J.~Yelton}\affil[21]{University of Florida, Gainesville, Florida 32611}


==> bibliography.tex <==
\begin{thebibliography}{99}

%Physics Case  References

\bibitem{BelleIITDR} 
T.~Abe {\em et al.} Belle II Technical Design Report, KEK Report 2010-1,
Edited by Z.~Dolezal and S.~Uno, arXiv:1011.0352 (2010).
\bibitem{LEPSLDReport2006} 
ALEPH and DELPHI and L3 and OPAL and SLD Collaborations and LEP Electroweak Working Group and SLD Electroweak Group and SLD Heavy Flavour Group (S. Schael et al.),
`` Precision electroweak measurements on the Z$^0$ resonance'', Phys.Rept. 427 (2006) 257-454.
\bibitem{SuperBTDR} M.~Baszczyk {\em et al.} (SuperB Collaboration), ``SuperB Technical Design Report'', INFN-13-01/PI, LAL 13-01, SLAC-R-1003,
 arXiv:1306.5655 [physics.ins-det].
\bibitem{Aleskejevs} A.~Aleksejevs, S.~Barkanova, C.~Miller, J.M.~Roney and V.~Zykunov,
``NLO Radiative Corrections for Forward-Backward and Left-Right Asymmetries at a B-Factory'', arXiv:1801.08510.
\bibitem{ErlerPDG2018} J.~Erler and A. Freitas ``ElectroweakModel and Constraints on New Physics'' 
 in M. Tanabashi {\em et al.} (Particle Data Group), Phys.~Rev.~D{\bf 98}, 030001 (2018);
 J.~Benesch {\em et al.} (Moller Collaboration), ``The MOLLER Experiment: An Ultra-Precise Measurement of the Weak Mixing Angle Using M{\o}ller Scattering'',
JLAB-PHY-14-1986, arXiv:1411.4088v2 [nucl-ex] 2014;
D.~ Becker {\em  et al.}  ``The P2 experiment'', arXiv:1802.04759 [nucl-ex] 2018.

\bibitem{UliWienands} Uli Wienands, private communication
\bibitem{Pospelov:2008jd} M.~Pospelov and A.~Ritz, ``Astrophysical Signatures of Secluded Dark Matter'', Phys. Lett. B671:391–397,
2009.
\bibitem{ArkaniHamed:2008qn} N.~Arkani-Hamed, D.~P.~Finkbeiner, T.~R.~Slatyer, and N.~Weiner, ``A Theory of Dark Matter'', Phys. Rev. D79:015014, 2009.
\bibitem{Batell:2011qq} B.~Batell, D.~McKeen, and M.~Pospelov,
``New Parity-Violating Muonic Forces and the Proton Charge Radius'', Phys.Rev.Lett. 107:011803, 2011.
arXiv:1103.0721 [hep-ph].
\bibitem{Pohl:2010zza} R.~Pohl, A.~Antognini, F.~Nez, F.~D.~Amaro, F.~Biraben, et al., ``The size of the proton'', Nature 466:213–216, 2010.
\bibitem{Davoudiasl} H.~Davoudiasl, H.~S.~Lee and W.~J.~Marciano, Phys.Rev. D 92, no. 5, 055005 (2015)

%BINP Spin Rotator References

\bibitem{Ohnishi-IPAC2011} Y. Ohnishi, H. Koiso, A. Morita, H. Sugimoto, and K. Oide, “LATTICE DESIGN OF LOW    EMITTANCE AND LOW BETA FUNCTION AT COLLISION POINT FOR SuperKEKB”, Proceedings of   IPAC2011, San Sebastián, Spain THPZ007.

\bibitem{Ohnishi-ICHEP2016} Y. Ohnishi on behalf of the SuperKEKB accelerator group, “Start of SuperKEKB”, 38th International Conference on High Energy Physics 3-10 August 2016 Chicago, USA. Published in PoS ICHEP2016 (2016) 006, pp.8.

\bibitem{Kuriki-JoP} Masao Kuriki and Kazunari Masaki 2019 J. Phys.: Conf. Ser. 1350 012047

\bibitem{Koop1}I. Koop, A. Otboev and Yu. Shatunov, “Issues and Challenges for Longitudinal Polarization  in SuperKEKB”, a talk given at BELLE-II Collaboration Meeting. February 2020, Tsukuba.

\bibitem{Wienands} U. Wienands, ANL-APS and N. Wang, U. of Illinois Urbana-Champaign (Lee Teng Student), “A   Compact Spin Rotator”, 24-Jun-2020, Belle 2 GM.

\bibitem{Zholents} A.A. Zholents, V.N. Litvinenko, Preprint YAF 81-80 (1981), also in DESY-L-TRANS-289.

\bibitem{Luijckx} G. Luijckx et al, “Polarized electrons in the AmPS storage ring”, Proc. of  PAC1997, Vancouver, Canada, 1997, pp.1063-1065.

\bibitem{Ptitsyn1} V.I. Ptitsyn, PhD thesis, Novosibirsk, 1997, in Russian. 

\bibitem{Ptitsyn2} V.I. Ptitsyn, Yu.M. Shatunov, S.R. Mane,” Spin response formalism in circular accelerators”, Nuclear Instruments and Methods in Physics Research A 608 (2009) 225–233.

\bibitem{Derbenev} Ya.S.Derbenev, A.M.Kondratenko, “Polarization kinematics of particles in storage rings”, Sov.Phys.JETP 37:968-973, 1973, Zh.Eksp.Teor.Fiz.64:1918-1929, 1973.


\bibitem{Koop2} I. A. Koop, A. V. Otboyev, P. Yu. Shatunov, and Yu. M. Shatunov, “Spin transparent Siberian Snake and Spin Rotator with solenoids”, SPIN-2006, Kyoto,  AIP Conference Proceedings 915, 948 (2007).

%ANL Spin Rotator References

\bibitem{decouple}Vladimir N. Litvinenko and Alexander A. Zholents.  Compensating effect of solenoids with quadrupole lenses. 1984.

\bibitem{direct-wind} Brett Parker, Michael Anerella, John Escallier, Arup Ghosh, Animesh Jain, Andrew Marone, Joseph Muratore, and Peter Wanderer. BNL Direct Wind Superconducting Magnets. IEEE Trans. Appl. Supercond., 22(3):4101604, 2012.

\bibitem{Yuhao} Yuhao Peng, Conceptual Design of the Spin Rotator for the SuperKEKB High Energy Ring, MSc Thesis, University of Victoria, 2021

\bibitem{BMAD} D. Sagan. The BMAD Reference Manual. https://www.classe.cornell.edu/
bmad/manual.html, 2021.

\bibitem{SAD} Demin Zhou, Maria Biagini, Nicola Carmignani, Haruyo Koiso, Simone Liuzzo, Akio Morita, Yukiyoshi Ohnishi, Katsunobu Oide, David Sagan, and Hiroshi Sugimoto. Lattice Translation Between Accelerator Simulation Codes for Superkekb. In 7th International Particle Accelerator Conference, page WEPOY040, 2016.


\bibitem{Cmat} D. Sagan and D. Rubin. Linear analysis of coupled lattices. Phys.Rev., 2(074001), 1999.

\bibitem{superkekb}Y. Suetsugu, H. Fukuma, K. Ohmi, M. Tobiyama, John Flanagan, Hirokazu Ikeda, Emy Mulyani, K. Shibata, T. Ishibashi, M. Shirai, Shinji Terui, KoujiKanazawa, and H. Hisamatsu. Mitigating the electron cloud effect in the superkekb positron ring. Physical Review Accelerators and Beams, 22, 02 2019.

\bibitem{wille} Klaus Wille. The physics of particle accelerators : an introduction. Oxford University Press, 2000.

\bibitem{kek}Kazunori Akai, Kazuro Furukawa, and Haruyo Koiso. Superkekb collider. Nuclear Instruments and Methods in Physics Research Section A: Accelerators,Spectrometers, Detectors and Associated Equipment, 907, 08 2018.


\bibitem{LTT}D. Sagan. Long Term Tracking Program. https://www.classe.cornell.edu/bmad/other\_manuals.html, 2021


%Polarimetry

\bibitem{HAGIWARArho}K.~Hagiwara, A.~Martin, D.~Zeppenfeld, $\tau$ polarization measurements at LEP and SLC. {\em Physics Letters B}. \textbf{235}, 198-202 (1990)

\bibitem{Barlow}R.~Barlow, C.~Beeston, Fitting using finite Monte Carlo samples. {\em Comput. Phys. Commun.}. \textbf{77} pp. 219-228 (1993)

%ALR
\bibitem{B2lumi} F.~Abudin{\'e}n, {\em et. al.},  Measurement of the integrated luminosity of the Phase 2 data of the Belle II experiment. {\em Chinese Physics C}. \textbf{44}, 021001 (2020,2)

\bibitem{AleksBhabha} Aleksejevs, A., Barkanova, S., Bystritskiy, Y. \& Zykunov, V. Electroweak Corrections with Allowance for Hard Bremsstrahlung in Polarized Bhabha Scattering. {\em Physics Of Atomic Nuclei}. \textbf{83}, 463-479 (2020,5), https://doi.org/10.1134/S1063778820030035

\bibitem{ReneSANCe} Sadykov, R. \& Yermolchyk, V. Polarized NLO EW e+e− cross section calculations with ReneSANCe-v1.0.0. {\em Computer Physics Communications}. \textbf{256} pp. 107445 (2020), https://www.sciencedirect.com/science/article/pii/S0010465520302083


\end{thebibliography}


